Method and System for Image Analysis to Detect Cancer

Breast cancer is the most common cancer and is the leading cause of cancer death among women worldwide. Detection of breast cancer, while it is still small and confined to the breast, provides the best chance of effective treatment. Computer Aided Detection (CAD) systems that detect cancer from mammograms will help in reducing the human errors that lead to missing breast carcinoma. Literature is rich of scientific papers for methods of CAD design, yet with no complete system architecture to deploy those methods. On the other hand, commercial CADs are developed and deployed only to vendors' mammography machines with no availability to public access. This paper presents a complete CAD; it is complete since it combines, on a hand, the rigor of algorithm design and assessment (method), and, on the other hand, the implementation and deployment of a system architecture for public accessibility (system). (1) We develop a novel algorithm for image enhancement so that mammograms acquired from any digital mammography machine look qualitatively of the same clarity to radiologists' inspection; and is quantitatively standardized for the detection algorithms. (2) We develop novel algorithms for masses and microcalcifications detection with accuracy superior to both literature results and the majority of approved commercial systems. (3) We design, implement, and deploy a system architecture that is computationally effective to allow for deploying these algorithms to cloud for public access.

==> SecConclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
This paper is the main publication of a project coined to design a complete Computer Aided Detection
(CAD) for detecting breast cancer from mammograms. The project involved several researchers from
several disciplines and a large database was acquired from two different institutions for design and
assessment. This CAD is complete since it is comprised of both method and system. The method is a
set of algorithms designed for image enhancement, mass detection, and microcalcification
detection. The system is an implementation and deployment of a software architecture that
facilitates both local and cloud access to the designed algorithms so that the CAD is not limited to
a particular or local mammography machine. The assessment results of both the method and the system
are presented. The results of method assessment illustrate that the CAD sensitivity is much higher
than the majority of commercial and FDA approved CADs. The results of system assessment illustrates
that the layer responsible for deploying the CAD to the cloud has a minimal effect on the CAD
performance, and that the majority of the delay comes from the algorithm computations.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Yousef2018CAD"
%%% End:

